Deep Reinforcement Learning for DER Cyber-Attack Mitigation

The increasing penetration of DER with smart-inverter functionality is set to transform the electrical distribution network from a passive system, with fixed injection/consumption, to an active network with hundreds of distributed controllers dynamically modulating their operating setpoints as a function of system conditions. This transition is being achieved through standardization of functionality through grid codes and/or international standards. DER, however, are unique in that they are typically neither owned nor operated by distribution utilities and, therefore, represent a new emerging attack vector for cyber-physical attacks. Within this work we consider deep reinforcement learning as a tool to learn the optimal parameters for the control logic of a set of uncompromised DER units to actively mitigate the effects of a cyber-attack on a subset of network DER.

==> tikz/voltage_analysis.tex <==
\newcommand{\errorband}[5][]{
\pgfplotstableread[col sep=comma]{#2}\datatable
  \addplot [name path=pluserror,draw=none,no markers,forget plot]
    table [x={#3},y expr=\thisrow{#4}+\thisrow{#5}] {\datatable};

  \addplot [name path=minuserror,draw=none,no markers,forget plot]
    table [x={#3},y expr=\thisrow{#4}-\thisrow{#5}] {\datatable};

  \addplot [forget plot, fill=gray!40, #1]
    fill between[on layer={},of=pluserror and minuserror];
}

\begin{tikzpicture}
\definecolor{tableau_blue}{RGB}{31,119,180}

\begin{axis}[
enlarge x limits=false,
try min ticks=3,
tick pos=left,
minor y tick num=1,
ymajorgrids=true,
yminorgrids=true,
%tick align=outside,
width=\linewidth,
height=\linewidth / 2,
xlabel=simulation steps (seconds),
ylabel=voltage]

\errorband[tableau_blue, opacity=0.2]{data/voltage_analysis.csv}{}{mean}{std}
\addplot [smooth, thick, tableau_blue, no markers] table [x=, y=mean, col sep=comma] {data/voltage_analysis.csv};

\end{axis}
\end{tikzpicture}
